Interpolative Butterfly Factorization

This paper introduces the interpolative butterfly factorization for nearly optimal implementation of several transforms in harmonic analysis, when their explicit formulas satisfy certain analytic properties and the matrix representations of these transforms satisfy a complementary low-rank property. A preliminary interpolative butterfly factorization is constructed based on interpolative low-rank approximations of the complementary low-rank matrix. A novel sweeping matrix compression technique further compresses the preliminary interpolative butterfly factorization via a sequence of structure-preserving low-rank approximations. The sweeping procedure propagates the low-rank property among neighboring matrix factors to compress dense submatrices in the preliminary butterfly factorization to obtain an optimal one in the butterfly scheme. For an $N\times N$ matrix, it takes $O(N\log N)$ operations and complexity to construct the factorization as a product of $O(\log N)$ sparse matrices, each with $O(N)$ nonzero entries. Hence, it can be applied rapidly in $O(N\log N)$ operations. Numerical results are provided to demonstrate the effectiveness of this algorithm.

==> figure/fig-comp-modules/fig-K.tex <==
\begin{tikzpicture}[baseline=-0.5ex]
      \tikzset{every left delimiter/.style={xshift=-1ex},every right delimiter/.style={xshift=1ex}}
      \matrix (mat) [matrix of math nodes, left delimiter=(, right delimiter=)] {
\draw[fill=gray] (0,0) rectangle (32,32);
\\
      };
\end{tikzpicture}

==> figure/fig-comp-modules/fig-comp-u1.tex <==
\begin{tikzpicture}[baseline=-0.5ex]
      \tikzset{every left delimiter/.style={xshift=-1ex},every right delimiter/.style={xshift=1ex}}
      \matrix (mat) [matrix of math nodes, left delimiter=(, right delimiter=)] {
\draw;
\foreach \k in {0,2,...,30}{
\foreach \i in {0,0.5,...,1.5} {
    \draw[fill=gray] (32-\i-\k,\k) rectangle (32-\i-\k-0.5,\k+2);
}
}\\
      };
\end{tikzpicture}

==> figure/fig-comp-modules/fig-comp-u2.tex <==
\begin{tikzpicture}[baseline=-0.5ex]
      \tikzset{every left delimiter/.style={xshift=-1ex},every right delimiter/.style={xshift=1ex}}
      \matrix (mat) [matrix of math nodes, left delimiter=(, right delimiter=)] {
\draw;
\foreach \k in {0,1,...,31}{
\foreach \i in {0,0.5} {
    \draw[fill=gray] (32-\i-\k,\k) rectangle (32-\i-\k-0.5,\k+1);
}
}\\
      };
\end{tikzpicture}

==> figure/fig-comp-modules/fig-comp-v1.tex <==
\begin{tikzpicture}[baseline=-0.5ex]
      \tikzset{every left delimiter/.style={xshift=-1ex},every right delimiter/.style={xshift=1ex}}
      \matrix (mat) [matrix of math nodes, left delimiter=(, right delimiter=)] {
\draw;
\foreach \k in {0,2,...,30}{
\foreach \i in {0,0.5,...,1.5} {
    \draw[fill=gray] (\k,32-\i-\k) rectangle (\k+2,32-\i-\k-0.5);
}
}\\
      };
\end{tikzpicture}

==> figure/fig-comp-modules/fig-comp-v2.tex <==
\begin{tikzpicture}[baseline=-0.5ex]
      \tikzset{every left delimiter/.style={xshift=-1ex},every right delimiter/.style={xshift=1ex}}
      \matrix (mat) [matrix of math nodes, left delimiter=(, right delimiter=)] {
\draw;
\foreach \k in {0,1,...,31}{
\foreach \i in {0,0.5} {
    \draw[fill=gray] (\k,32-\i-\k) rectangle (\k+1,32-\i-\k-0.5);
}
}\\
      };
\end{tikzpicture}

==> figure/fig-compression-1D.tex <==
\begin{figure}[htp]
\begin{minipage}{\textwidth}
\centering
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-K}
}
$\approx$
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-uncomp-u}
}
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-M}
}
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-uncomp-v}
}\\
\end{minipage}
\caption{The middle level factorization of
    a $64\times 64$ complementary low-rank matrix $\tilde{M}^h\approx C^3M^3(R^3)^*$
    assuming $r=1$.
    Grey blocks indicate nonzero blocks.
    $C^3$ and $R^3$ are block-diagonal matrices with $8$ blocks.
    The diagonal blocks of $C^3$ and $R^3$ are assembled
    according to Equation \eqref{eq:expression-UV}
    as indicated by black rectangles.
    $M^3$ is a $8\times 8$ block matrix with each block
    $M^3_{i,j}$ itself an $8\times 8$ block matrix
    containing diagonal weights matrix on the $(j,i)$ block.}
\label{fig:compression-1D}
\end{figure}


==> figure/fig-compression-1D2.tex <==
\begin{figure}[htp]
\begin{minipage}{\textwidth}
\centering
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-uncomp-u2}
}
$\approx$
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-uncomp-svd}
}
=
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-comp-u1}
}
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-comp-g1}
}\\
\resizebox{3.5cm}{!}{
}
$\approx$
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-comp-u2}
}
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-comp-g2}
}
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-comp-g1}
}\\
\end{minipage}
\caption{The recursive factorization of $U^3$
    in Figure~\ref{fig:compression-1D}.
    Gray factors are matrices inheriting the complementary low-rank
    property.
    Top: left matrix: $U^3$ with each diagonal block
    partitioned into smaller blocks according to
    Equation \eqref{eqn:half} as indicated by black rectangles;
    middle-left matrix: low-rank approximations of submatrices
    in $U^3$ given by Equation \eqref{eqn:RSh};
    middle right matrix: $U^4$;
    right matrix: $G^3$.
    Bottom: $U^4$ in the first row is further factorized into
    $U^4\approx U^5G^4$, giving $U^3 \approx U^5 G^4 G^3$.}
\label{fig:compression-1D2}
\end{figure}

==> figure/fig-compression-1D3.tex <==
\begin{figure}[htp]
\begin{minipage}{\textwidth}
\centering
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-uncomp-v2}
}
=
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-comp-h1}
}
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-comp-h2}
}
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-comp-v2}
}\\
\end{minipage}
\caption{The recursive factorization $(V^3)^* \approx (H^3)^*(H^4)^*(V^5)^*$ of $(V^3)^*$
    in Figure~\ref{fig:compression-1D}.}
\label{fig:compression-1D3}
\end{figure}


==> figure/fig-domain-tree-BF.tex <==
\begin{figure}
\centering
\begin{tikzpicture}[scale=0.3]

\draw [->,double,double distance=1pt] (-6,5.5) -> (-6,10);

\draw [->,double,double distance=1pt] (-6,4.5) -> (-6,0);

\draw (0,10) -- (-4,0) -- (4,0) -- cycle;

\draw [->,double,double distance=1pt] (20,5.5) -> (20,10);

\draw [->,double,double distance=1pt] (20,4.5) -> (20,0);

\draw (14,10) -- (10,0) -- (18,0) -- cycle;

\draw [latex-latex,line width=1pt] (9,5) -> (5,5);
\draw [latex-latex,line width=1pt] (9,9) -> (5,1);
\draw [latex-latex,line width=1pt] (9,1) -> (5,9);

\coordinate [label=above:$T_X$] (X) at (0,10);
\coordinate [label=above:$T_\Omega$] (X) at (14,10);

\draw (-2,5) -- (2,5);
\draw (12,5) -- (16,5);

\coordinate [label=right:$\frac{L}{2}$] (X) at (16,5);
\coordinate [label=left:$\frac{L}{2}$] (X) at (-2,5);
\end{tikzpicture}
\caption{Trees of the row and column indices.
    Left: $T_X$ for the row indices $X$.
    Right: $T_\Omega$ for the column indices $\Omega$.
    The interaction between $A\in T_X$ and $B\in T_\Omega$
    starts at the middle level of $T_X$ and the leaves of 
    $T_\Omega$ for the middle level factorization. The 
    interaction goes down in $T_X$ and goes up in $T_\Omega$ 
    simultaneously for the recursive factorization of 
    left factors. The interaction goes up in $T_X$ and 
    goes down in $T_\Omega$ 
    simultaneously for the recursive factorization of 
    right factors. }
\label{fig:domain-tree-BF}
\end{figure}

==> figure/fig-double-block-matrix.tex <==
\begin{figure}[htp]
\begin{minipage}{0.32\textwidth}
\begin{tikzpicture}[scale=0.25]
\draw[draw=black] (0,0) rectangle (16,16);
\draw[draw=black,dashed] (0,8) rectangle (16,12);
\draw[draw=black,dashed] (8,0) rectangle (12,16);
\draw[draw=black] (8,8) rectangle (12,12);
\draw[draw=black,dashed] (9,8) rectangle (10,12);
\draw[draw=black,dashed] (8,9) rectangle (12,10);
\filldraw[fill=lightgray,draw=black] (9,9) rectangle (10,10);
\draw (0,10) node[left=3pt,rectangle,fill=white] {$A$};
\draw (10,16) node[above=3pt,rectangle,fill=white] {$B$};
\draw (8,9.5) node[left=3pt,rectangle,fill=white] {{\tiny $C$}};
\draw (9.5,12) node[above=3pt,rectangle,fill=white] {{\tiny $D$}};
\draw (8,0) node[below=5pt,rectangle,fill=white] {$M_{AB,CD}$};
\end{tikzpicture}
\end{minipage}
\caption{The visualization of the submatrices $\{M_{AB,CD}\}$, $\{M_{AB,:D}\}$, and $\{M_{AB,C:}\}$ in $M_{AB}$. The largest black rectangle represents a matrix $M$ and the smaller one inside $M$ indicates its submatrix $M_{AB}$. From left to right, the light gray boxes inside $M_{AB}$ indicate the submatrices  $\{M_{AB,CD}\}$, $\{M_{AB,:D}\}$, and $\{M_{AB,C:}\}$, respectively.}
\label{fig:double-block-matrix}
\end{figure}
